Simultaneous Confidence Bands for Functional Data Using the Gaussian Kinematic Formula

This article constructs simultaneous confidence bands (SCBs) for functional parameters using the Gaussian Kinematic formula of $t$-processes (tGKF). Although the tGKF relies on Gaussianity, we show that a central limit theorem (CLT) for the parameter of interest is enough to obtain asymptotically precise covering rates even for non-Gaussian processes. As a proof of concept we study the functional signal-plus-noise model and derive a CLT for an estimator of the Lipschitz-Killing curvatures, the only data dependent quantities in the tGKF SCBs. Extensions to discrete sampling with additive observation noise are discussed using scale space ideas from regression analysis. Here we provide sufficient conditions on the processes and kernels to obtain convergence of the functional scale space surface. The theoretical work is accompanied by a simulation study comparing different methods to construct SCBs for the population mean. We show that the tGKF works well even for small sample sizes and only a Rademacher multiplier-$t$ bootstrap performs similarily well. For larger sample sizes the tGKF often outperforms the bootstrap methods and is computational faster. We apply the method to diffusion tensor imaging (DTI) fibers using a scale space approach for the difference of population means. R code is available in our Rpackage SCBfda.

==> references.tex <==
@booktitle{Adler1981,
  title={The geometry of random fields},
  author={Adler, Robert J},
  volume={62},
  year={1981},
  publisher={Siam}
}
@article{Adler2000,
  title={On excursion sets, tube formulas and maxima of random fields},
  author={Adler, Robert J},
  journal={The Annals of Applied Probability},
  volume={10},
  number={1},
  pages={1--74},
  year={2000},
  publisher={JSTOR}
}
@booktitle{Adler2007,
  title={Random fields and geometry},
  author={Adler, Robert J and Taylor, Jonathan E},
  year={2007},
  publisher={Springer Science \& Business Media}
}
@article{Adler2017,
  title={Estimating thresholding levels for random fields via Euler characteristics},
  author={Adler, Robert J and Bartz, Kevin and Kou, Sam C and Monod, Anthea},
  journal={arXiv preprint arXiv:1704.08562},
  year={2017}
}
@article{Belloni2018,
  title={Uniformly valid post-regularization confidence regions for many functional parameters in z-estimation framework},
  author={Belloni, Alexandre and Chernozhukov, Victor and Chetverikov, Denis and Wei, Ying and others},
  journal={The Annals of Statistics},
  volume={46},
  number={6B},
  pages={3643--3675},
  year={2018},
  publisher={Institute of Mathematical Statistics}
}
@article{Bunea2011,
  title={Adaptive inference for the mean of a Gaussian process in functional data},
  author={Bunea, Florentina and Ivanescu, Andrada E and Wegkamp, Marten H},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={73},
  number={4},
  pages={531--558},
  year={2011},
  publisher={Wiley Online Library}
}
@article{Cai2011,
  title={Optimal estimation of the mean function based on discretely sampled functional data: Phase transition},
  author={Cai, T Tony and Yuan, Ming},
  journal={The annals of statistics},
  pages={2330--2355},
  year={2011},
  publisher={JSTOR}
}
@article{Cao1999,
  title={The detection of local shape changes via the geometry of Hotelling's ${T}^2$ fields},
  author={Cao, Jin and Worsley, Keith J and others},
  journal={The Annals of Statistics},
  volume={27},
  number={3},
  pages={925--942},
  year={1999},
  publisher={Institute of Mathematical Statistics}
}
@article{Cao2012,
  title={Simultaneous inference for the mean function based on dense functional data},
  author={Cao, Guanqun and Yang, Lijian and Todem, David},
  journal={Journal of Nonparametric Statistics},
  volume={24},
  number={2},
  pages={359--377},
  year={2012},
  publisher={Taylor \& Francis}
}
@article{Cao2014,
  title={Simultaneous confidence bands for derivatives of dependent functional data},
  author={Cao, Guanqun and others},
  journal={Electronic Journal of Statistics},
  volume={8},
  number={2},
  pages={2639--2663},
  year={2014},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{Chaudhuri2000,
  title={Scale space view of curve estimation},
  author={Chaudhuri, Probal and Marron, James Steven},
  journal={Annals of Statistics},
  pages={408--428},
  year={2000},
  publisher={JSTOR}
}
@article{Chaudhuri1999,
  title={SiZer for exploration of structures in curves},
  author={Chaudhuri, Probal and Marron, James S},
  journal={Journal of the American Statistical Association},
  volume={94},
  number={447},
  pages={807--823},
  year={1999},
  publisher={Taylor \& Francis}
}
@article{Chang2017,
  title={Simultaneous confidence bands for functional regression models},
  author={Chang, Chung and Lin, Xuejing and Ogden, R Todd},
  journal={Journal of Statistical Planning and Inference},
  volume={188},
  pages={67--81},
  year={2017},
  publisher={Elsevier}
}
@article{Chernozhukov2013,
  title={Gaussian approximations and multiplier bootstrap for maxima of sums of high-dimensional random vectors},
  author={Chernozhukov, Victor and Chetverikov, Denis and Kato, Kengo and others},
  journal={The Annals of Statistics},
  volume={41},
  number={6},
  pages={2786--2819},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{Chiani2003,
  title={New exponential bounds and approximations for the computation of error probability in fading channels},
  author={Chiani, Marco and Dardari, Davide and Simon, Marvin K},
  journal={IEEE Transactions on Wireless Communications},
  volume={2},
  number={4},
  pages={840--845},
  year={2003},
  publisher={IEEE}
}
@article{Chen2017,
  title={Density level sets: Asymptotics, inference, and visualization},
  author={Chen, Yen-Chi and Genovese, Christopher R and Wasserman, Larry},
  journal={Journal of the American Statistical Association},
  pages={1--13},
  year={2017},
  publisher={Taylor \& Francis}
}
@article{Crainiceanu2011,
  title={Statistical inference on the difference in the means of two correlated functional processes: an application to sleep EEG power spectra},
  author={Crainiceanu, Ciprian M and Staicu, Ana-Maria and Ray, Shubankar and Punjabi, Naresh},
  journal={Johns Hopkins University, Dept. of Biostatistics Working Papers},
  pages={225},
  year={2011},
  publisher={bepress}
}
@article{Cuevas2006,
  title={On the use of the bootstrap for estimating functions with functional data},
  author={Cuevas, Antonio and Febrero, Manuel and Fraiman, Ricardo},
  journal={Computational statistics \& data analysis},
  volume={51},
  number={2},
  pages={1063--1074},
  year={2006},
  publisher={Elsevier}
}
@article{Cuevas2014,
  title={A partial overview of the theory of statistics with functional data},
  author={Cuevas, Antonio},
  journal={Journal of Statistical Planning and Inference},
  volume={147},
  pages={1--23},
  year={2014},
  publisher={Elsevier}
}
@booktitle{Davidson1994,
  title={Stochastic Limit Theory: An introduction for econometricians},
  author={Davidson, James},
  year={1994},
  publisher={OUP Oxford}
}
@article{Davidson2008,
  title={The wild bootstrap, tamed at last},
  author={Davidson, Russell and Flachaire, Emmanuel},
  journal={Journal of Econometrics},
  volume={146},
  number={1},
  pages={162--169},
  year={2008},
  publisher={Elsevier}
}

@article{Deng2017,
  title={Beyond Gaussian approximation: bootstrap for maxima of sums of independent random vectors},
  author={Deng, Hang and Zhang, Cun-Hui},
  journal={arXiv preprint arXiv:1705.09528},
  volume={},
  number={},
  pages={},
  year={2017}
}

@article{DelBarrio2015,
  title={A statistical analysis of a deformation model with Wasserstein barycenters: estimation procedure and goodness of fit test},
  author={Del Barrio, Eustasio and H{\'e}l{\`e}ne, Lescornel and Jean-Michel, Loubes},
  journal={arXiv preprint arXiv:1508.06465},
  year={2015}
}
@article{Degras2011,
  title={Simultaneous confidence bands for nonparametric regression with functional data},
  author={Degras, David A},
  journal={Statistica Sinica},
  volume={21},
  number={4},  
  pages={1735--1765},
  year={2011},
  publisher={JSTOR}
}
@article{Degras2017,
  title={Simultaneous confidence bands for the mean of functional data},
  author={Degras, David},
  journal={Wiley Interdisciplinary Reviews: Computational Statistics},
  volume={9},
  number={3},
  year={2017},
  publisher={Wiley Online Library}
}
@article{Ciccio1996,
  title={Bootstrap confidence intervals},
  author={DiCiccio, Thomas J and Efron, Bradley},
  journal={Statistical science},
  pages={189--212},
  year={1996},
  publisher={JSTOR}
}
@article{Ferreira2012,
  title={Reproducing properties of differentiable Mercer-like kernels},
  author={Ferreira, Jos{\'e} C and Menegatto, Valdir A},
  journal={Mathematische Nachrichten},
  volume={285},
  number={8-9},
  pages={959--973},
  year={2012},
  publisher={Wiley Online Library}
}
@article{Goldsmith2013,
  title={Corrected confidence bands for functional data using principal components},
  author={Goldsmith, Jeff and Greven, Sonja and Crainiceanu, CIPRIAN},
  journal={Biometrics},
  volume={69},
  number={1},
  pages={41--51},
  year={2013},
  publisher={Wiley Online Library}
}
@booktitle{Good2005,
  title={Permutation, parametric and bootstrap tests of hypotheses: a practical guide to resampling methods for testing hypotheses},
  author={Good, Phillip I},
  year={2005},
  publisher={Springer Science \& Business Media}
}
@article{Hahn1977,
  title={Conditions for sample-continuity and the central limit theorem},
  author={Hahn, Marjorie G},
  journal={The Annals of Probability},
  pages={351--360},
  year={1977},
  publisher={JSTOR}
}
@article{Hall2006,
  title={Properties of principal component methods for functional and longitudinal data analysis},
  author={Hall, Peter and M{\"u}ller, Hans-Georg and Wang, Jane-Ling},
  journal={The annals of statistics},
  pages={1493--1517},
  year={2006},
  publisher={JSTOR}
}
@article{Hall2007,
  title={Two-sample tests in functional data analysis starting from discrete data},
  author={Hall, Peter and Van Keilegom, Ingrid},
  journal={Statistica Sinica},
  pages={1511--1531},
  year={2007},
  publisher={JSTOR}
}
@article{Hart1993,
  title={Consistency of cross-validation when the data are curves},
  author={Hart, Jeffrey D and Wehrly, Thomas E},
  journal={Stochastic processes and their applications},
  volume={45},
  number={2},
  pages={351--361},
  year={1993},
  publisher={Elsevier}
}

@article{Horvath2009,
  title={Two sample inference in functional linear models},
  author={Horv{\'a}th, Lajos and Kokoszka, Piotr and Reimherr, Matthew},
  journal={Canadian Journal of Statistics},
  volume={37},
  number={4},
  pages={571--591},
  year={2009},
  publisher={Wiley Online Library}
}
@booktitle{Hsing2015,
  title={Theoretical foundations of functional data analysis, with an introduction to linear operators},
  author={Hsing, Tailen and Eubank, Randall},
  year={2015},
  publisher={John Wiley \& Sons}
}

@article{Jain1975,
  title={Central limit theorems for C (S)-valued random variables},
  author={Jain, Naresh C and Marcus, Michael B},
  journal={Journal of Functional Analysis},
  volume={19},
  number={3},
  pages={216--231},
  year={1975},
  publisher={Elsevier}
}

@article{Johansen1990,
  title={Hotelling's theorem on the volume of tubes: some illustrations in simultaneous inference and data analysis},
  author={Johansen, Soren and Johnstone, Iain M},
  journal={The Annals of Statistics},
  volume={18},
  number={2},
  pages={652--684},
  year={1990},
  publisher={JSTOR}
}
@article{Kuriki2001,
  title={Tail probabilities of the maxima of multilinear forms and their applications},
  author={Kuriki, Satoshi and Takemura, Akimichi},
  journal={Annals of statistics},
  pages={328--371},
  year={2001},
  publisher={JSTOR}
}
@booktitle{Kosorok2008,
  title={Introduction to empirical processes and semiparametric inference.},
  author={Kosorok, Michael R},
  year={2008},
  publisher={Springer}
}
@article{Krivobokova2010,
  title={Simultaneous confidence bands for penalized spline estimators},
  author={Krivobokova, Tatyana and Kneib, Thomas and Claeskens, Gerda},
  journal={Journal of the American Statistical Association},
  volume={105},
  number={490},
  pages={852--863},
  year={2010},
  publisher={Taylor \& Francis}
}
@article{LeBrigant2018,
  title={A discrete framework to find the optimal matching between manifold-valued curves},
  author={Le Brigant, Alice},
  journal={Journal of Mathematical Imaging and Vision},
  pages={1--31},
  year={2018},
  publisher={Springer}
}
@article{landau1970,
  title={On the supremum of a Gaussian process},
  author={Landau, HJ and Shepp, Lawrence A},
  journal={Sankhy{\=a}: The Indian Journal of Statistics, Series A},
  pages={369--378},
  year={1970},
  publisher={JSTOR}
}
@booktitle{Ledoux1991,
  title={Probability in Banach spaces, volume 23 of Ergebnisse der Mathematik und ihrer Grenzgebiete (3)[Results in Mathematics and Related Areas (3)]},
  author={Ledoux, Michel and Talagrand, Michel},
  year={1991},
  publisher={Springer-Verlag, Berlin}
}
@article{Li2010,
  title={Uniform convergence rates for nonparametric regression and principal component analysis in functional/longitudinal data},
  author={Li, Yehua and Hsing, Tailen and others},
  journal={The Annals of Statistics},
  volume={38},
  number={6},
  pages={3321--3351},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}
@article{Lu2017,
  title={Simultaneous confidence bands for contrasts between several nonlinear regression curves},
  author={Lu, Xiaolei and Kuriki, Satoshi},
  journal={Journal of Multivariate Analysis},
  volume={155},
  pages={83--104},
  year={2017},
  publisher={Elsevier}
}
@article{Mammen1993,
  title={Bootstrap and wild bootstrap for high dimensional linear models},
  author={Mammen, Enno},
  journal={The Annals of Statistics},
  volume={21},
  number={1},
  pages={255--285},
  year={1993},
  publisher={JSTOR}
}
@booktitle{Mardia1979,
  title={Multivariate analysis},
  author={Bibby, JM and Kent, JT and Mardia, KV},
  year={1979},
  publisher={Academic Press, London}
}
@article{Ostrovsky2013,
  title={CLT for continuous random processes under approximations terms},
  author={Ostrovsky, E and Sirota, L},
  journal={arXiv preprint arXiv:1304.0250},
  year={2013}
}
@article{Park2008,
  title={SiZer analysis for the comparison of regression curves},
  author={Park, Cheolwoo and Kang, Kee-Hoon},
  journal={Computational Statistics \& Data Analysis},
  volume={52},
  number={8},
  pages={3954--3970},
  year={2008},
  publisher={Elsevier}
}
@article{Park2014,
  title={Nonparametric comparison of multiple regression curves in scale-space},
  author={Park, Cheolwoo and Hannig, Jan and Kang, Kee-Hoon},
  journal={Journal of Computational and Graphical Statistics},
  volume={23},
  number={3},
  pages={657--677},
  year={2014},
  publisher={Taylor \& Francis}
}
@booktitle{Pollard1990,
  title={Empirical processes: theory and applications},
  author={Pollard, David},
  pages={i--86},
  year={1990},
  organization={JSTOR}
}
@booktitle{Ramsay2006,
  title={Functional data analysis},
  author={Ramsay, James O},
  year={2006},
  publisher={Wiley Online Library}
}
@article{Sommerfeld2015,
  title={Confidence regions for excursion sets in asymptotically Gaussian random fields, with an application to climate},
  author={Sommerfeld, Max and Sain, Stephen and Schwartzman, Armin},
  journal={arXiv preprint arXiv:1501.07000},
  year={2015}
}
@article{Schwartzmann2018,
 title={Estimation of Expected Euler Characteristic Curves of Nonstationary Gaussian Random Fields},
 author={Schwartzman, Armin and Cheng, Dan and Pranav, Pratyush and Adler, Robert},
  journal={arXiv preprint arXiv:1501.07000},
  year={2018}
}
@article{Taylor2005,
  title={Validity of the expected Euler characteristic heuristic},
  author={Taylor, Jonathan and Takemura, Akimichi and Adler, Robert J},
  journal={Annals of Probability},
  pages={1362--1396},
  year={2005},
  publisher={JSTOR}
}

@article{Takemura2002,
  title={On the equivalence of the tube and Euler characteristic methods for the distribution of the maximum of Gaussian fields over piecewise smooth domains},
  author={Takemura, Akimichi and Kuriki, Satoshi},
  journal={Annals of Applied Probability},
  pages={768--796},
  year={2002},
  publisher={JSTOR}
}
@article{Taylor2003,
  title={Euler characteristics for Gaussian fields on manifolds},
  author={Taylor, Jonathan E and Adler, Robert J},
  journal={Annals of Probability},
  pages={533--563},
  year={2003},
  publisher={JSTOR}
}
@article{Taylor2006,
  title={A Gaussian kinematic formula},
  author={Taylor, Jonathan E},
  journal={The Annals of Probability},
  volume={34},
  number={1},
  pages={122--158},
  year={2006},
  publisher={Institute of Mathematical Statistics}
}
@article{Taylor2009,
  title={Gaussian processes, kinematic formulae and Poincar{\'e}’s limit},
  author={Taylor, Jonathan E and Adler, Robert J and others},
  journal={The Annals of Probability},
  volume={37},
  number={4},
  pages={1459--1482},
  year={2009},
  publisher={Institute of Mathematical Statistics}
}
@article{TaylorWorsley2007,
  title={Detecting sparse signals in random fields, with an application to brain mapping},
  author={Taylor, Jonathan E and Worsley, Keith J},
  volume={102},
  number={479},
  pages={913--928},
  year={2007},
  publisher={Taylor \& Francis},
  journal={Journal of the American Statistical Association},
}
@article{Travis2015,
  title={Abnormal white matter properties in adolescent girls with anorexia nervosa},
  author={Travis, Katherine E and Golden, Neville H and Feldman, Heidi M and Solomon, Murray and Nguyen, Jenny and Mezer, Aviv and Yeatman, Jason D and Dougherty, Robert F},
  journal={NeuroImage: Clinical},
  volume={9},
  pages={648--659},
  year={2015},
  publisher={Elsevier}
}
@booktitle{Ledoux2013,
  title={Probability in Banach Spaces: isoperimetry and processes},
  author={Ledoux, Michel and Talagrand, Michel},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@article{Theil1965,
  title={The analysis of disturbances in regression analysis},
  author={Theil, Henri},
  journal={Journal of the American Statistical Association},
  volume={60},
  number={312},
  pages={1067--1079},
  year={1965},
  publisher={Taylor \& Francis}
}
@article{Zhang2007,
  title={Statistical inferences for functional data},
  author={Zhang, Jin-Ting and Chen, Jianwei and others},
  journal={The Annals of Statistics},
  volume={35},
  number={3},
  pages={1052--1079},
  year={2007},
  publisher={Institute of Mathematical Statistics}
}
@article{Zhang2016,
  title={From sparse to dense functional data and beyond},
  author={Zhang, Xiaoke and Wang, Jane-Ling and others},
  journal={The Annals of Statistics},
  volume={44},
  number={5},
  pages={2281--2321},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}
@article{Wang2016,
  title={Functional data analysis},
  author={Wang, Jane-Ling and Chiou, Jeng-Min and M{\"u}ller, Hans-Georg},
  journal={Annual Review of Statistics and Its Application},
  volume={3},
  pages={257--295},
  year={2016},
  publisher={Annual Reviews}
}
@article{Working1929,
  title={Applications of the theory of error to the interpretation of trends},
  author={Working, Holbrook and Hotelling, Harold},
  journal={Journal of the American Statistical Association},
  volume={24},
  number={165A},
  pages={73--85},
  year={1929},
  publisher={Taylor \& Francis}
}
@article{Worsley1994,
  title={Local maxima and the expected Euler characteristic of excursion sets of $\chi$ 2, F and t fields},
  author={Worsley, Keith J},
  journal={Advances in Applied Probability},
  volume={26},
  number={1},
  pages={13--42},
  year={1994},
  publisher={Cambridge University Press}
}
@article{Worsley1996,
  title={A unified statistical approach for determining significant signals in images of cerebral activation},
  author={Worsley, Keith J and Marrett, Sean and Neelin, Peter and Vandal, Alain C and Friston, Karl J and Evans, Alan C and others},
  journal={Human brain mapping},
  volume={4},
  number={1},
  pages={58--73},
  year={1996},
  publisher={Citeseer}
}
@article{Worsley2004,
  title={Unified univariate and multivariate random field theory},
  author={Worsley, Keith J and Taylor, Jonathan E and Tomaiuolo, Francesco and Lerch, Jason},
  journal={Neuroimage},
  volume={23},
  pages={S189--S195},
  year={2004},
  publisher={Elsevier}
}

